FedGTST: Boosting Global Transferability of Federated Models via Statistics Tuning

The performance of Transfer Learning (TL) heavily relies on effective pretraining, which demands large datasets and substantial computational resources. As a result, executing TL is often challenging for individual model developers. Federated Learning (FL) addresses these issues by facilitating collaborations among clients, expanding the dataset indirectly, distributing computational costs, and preserving privacy. However, key challenges remain unresolved. First, existing FL methods tend to optimize transferability only within local domains, neglecting the global learning domain. Second, most approaches rely on indirect transferability metrics, which do not accurately reflect the final target loss or true degree of transferability. To address these gaps, we propose two enhancements to FL. First, we introduce a client-server exchange protocol that leverages cross-client Jacobian (gradient) norms to boost transferability. Second, we increase the average Jacobian norm across clients at the server, using this as a local regularizer to reduce cross-client Jacobian variance. Our transferable federated algorithm, termed FedGTST (Federated Global Transferability via Statistics Tuning), demonstrates that increasing the average Jacobian and reducing its variance allows for tighter control of the target loss. This leads to an upper bound on the target loss in terms of the source loss and source-target domain discrepancy. Extensive experiments on datasets such as MNIST to MNIST-M and CIFAR10 to SVHN show that FedGTST outperforms relevant baselines, including FedSR. On the second dataset pair, FedGTST improves accuracy by 9.8% over FedSR and 7.6% over FedIIR when LeNet is used as the backbone.

==> Analysis.tex <==
\section{Sufficient Conditions on FL to promote domain transferability}


% LEMMA: General federated upper bound
\begin{lemma}[General federated loss upper bound]
\label{lem:gnr-fed-ub}
Assume that $l:\gW_h\times\gP_{\gX\times\gY}\to \sR_+$ is convex w.r.t. $w_{h}$. 
\begin{align*}
    L_{\gD_S}(h_S^{(0)})\leq \sE_{k\in[K]}\big[L_{\gD_S^{(k)}}\big(h_S^{(k)}\big)\big] + \overline{d}_{\gH}(\gD_S),
\end{align*}
where $\overline{d}_{\gH}(\gD_S):= \sE_{i,j\in[K]}d_{\gH}(\gD_S^{(i)}, \gD_S^{(j)})$.
\end{lemma}

\textit{Proof provided in Appendix.}\\\\
\textbf{Interpretation.} The LHS is the loss of the federated model, which is upper bounded by the RHS: the first term is the averaged local loss given by local models; The second term measures the averaged  local $\gH$-dependent divergence of the federated source domain. We remark that 
\begin{itemize}
    \item When the local domains are of i.i.d. distribution, we have $ L_{\gD_S}(h_S^{(0)})\leq \sE_{k\in[K]}\big[L_{\gD_S^{(k)}}\big(h_S^{(k)}\big)\big]$, which indicates that federated loss of federated model is upper bounded by the mean of local loss given local models.
    \item Suppose there are two function classes $\gH_2\subset\gH_1$, where $h_S^{(i)}\in\gH_1$, $h_S^{(i)}\in\gH_2$, $\forall i\in\{0\}\bigcup [K]$. Then the upper bound given training on $\gH_2$ is tighter than that training on $\gH_1$, which is equivalent to say, proper regularization decreasing the expressive capacity of $\gH$ leads to a tighter bound. 
\end{itemize} 
\Eve{todo: discuss realistic cases where l is convex w.r.t. w, i.e. Convolutional Neural Network (CNN), any model with Relu activation combined with linear or quadratic loss (MSE), etc.}

% Theorem: General transfer upper bound
\begin{theorem}
\label{thm:gen-tsf-fed-ub}
Suppose that $l$ is convex w.r.t. the weights $w_h$ of the model $h$.
\begin{align*}
    L_{\gD_T}(g_T\circ f_S^{(0)})\leq \sE_{k\in[K]}\big[L_{\gD_S^{(k)}}\big(h_S^{(k)}\big)\big] + \overline{d}_{\gH}(\gD_S) + d_{\gF}(\gD_S, \gD_T)
\end{align*}
where $\overline{d}_{\gH}(\gD_S):= \sE_{i,j\in[K], i\neq j}d_{\gH}(\gD_S^{(i)}, \gD_S^{(j)})$.
\end{theorem}

\textit{Proof obvious by combining Lemma \ref{lem:gen-tsf-ub} and \ref{lem:gnr-fed-ub}}\\\\
\textbf{Interpretation.} The target loss is upper bounded by the averaged loss of source local models, the $\gH-$dependent source local domain divergence, and the $\gF-$dependent transfer divergence between the source and target domain.\\\\
\textbf{Sufficient conditions.} (1) Proper regularization on the model function class $\gH$ during pre-training can tighten the upper bound (by lower the local divergence term). (2) lower averaged local loss given by local models tighten the upper bound.

Theorem \ref{thm:gen-tsf-fed-ub} provides generally sufficient conditions for promoting the transferability of a federated-trained model. However, to obtain specific inspiration for practice from theoretical analysis, we may tackle more specific settings and explore specific instructions for practical training techniques. Therefore, we further explore a more specific case. 



==> Experiment.tex <==
\section{Evaluation}
\subsection{Experimental Setting}
% We currently aim to attack the FRL framework given by Fan, Xiaofeng, et al.~\cite{bhagoji2019analyzing}.
\textbf{Individual agents: reinforcement learning.} We train our individual-agent model with two reinforcement learning algorithms: Vanilla Policy Gradient (VPG) and Proxy Policy Optimization (PPO)~\cite{schulman2017proximal}. We train on four OpenGYM environments: CartPole, Inverted Pendulum, Hopper, and Half Cheetah. For the VPG setting, the malicious agent attacks the reward with a budget of $\eps = 1$ and $\eps = 100$ to represent small-budget cases and large-budget cases. With a budget of $1$, each individual agent runs $100$ local steps without specified; For the PPO setting, the malicious agent attacks the reward with a budget of $100$, and each local agent runs $1000$ local steps. Other settings are as follows\footnote{These settings are inherited from the single-agent poisoning (\url{https://github.com/umd-huang-lab/poison-rl}).}: the attack cost is measured by $l2-$distance between the poisoned reward and the ground-truth observed reward. During each local training step, the maximum number of steps for termination is 300 if not restricted by the environment, the learning rate is 0.001 and the discount parameter is set to 0.99.
\\\\\textbf{Central server: federated training.} For the VPG setting, we run 100 communication rounds without specified for the small budget scenario ($\eps$ = 1) and run 1000 communication rounds for the large budget scenario ($\eps = 100$). For PPO setting, we run 1000 communication rounds. We use the conventional federate framework: the central server aggregates the models updated by local agents by taking the average at the end of each communication rounds, and then broadcasts the aggregated model to initialize the local agents' next round of local training.
\\\\\textbf{Generalization.} For VPG with a small attack budget ($\eps = 1$), we scale up the number of agents while keeping the proportion of malicious agents fixed. 
\\\\\textbf{Defense.} The naive defense protocol is added at the coordinator's aggregation step. For each updated model, We test it for $10$ episodes and use the mean reward per episode as its weight for aggregation. The weights are 

\subsection{Poisoning Federated Reinforcement Learning.}

\textbf{Baselines.} To the best of our knowledge, there's no study regarding poisoning FRL, therefore, we use clean training as the baseline.
\\\\\textbf{Performance.} VPG: small budget and a large budget; PPO: report the smallest portion.
\begin{figure}[t]
    % \vspace{-2.0em}
    \centering
    \includegraphics[height=3.4in]{figs/poison_vpg_f1.png}
    \includegraphics[height=1.85in]{figs/poison_ppo_f1.png}
    % \includegraphics[height=1.3in]{figs/figcifar-lastnorm.pdf}
    % \includegraphics[height=1.3in]{figs/figimagenet-lastnorm.pdf}
    % \caption{Robustness and transferability by controlling the norm of last layer with different approaches and parameters.\xiaojun{make caption clear, different parameter}}
    \vspace{-1em}
    % \caption{Relationship between robustness and transferability under different norms of last layer, via training with last-layer regularization (LLR) and last-layer orthogonalization (LLOT) %\sk{I suggest adding some interpretation, e.g., "plot indicates high negative correlation between bla and bla" }. \xiaojun{i feel it redundant if we add the same conclusion for all figures. what do you think?}
    % }
    \label{fig:result-ll}
    % \vspace{-1.5em}
\end{figure}
\\\\\textbf{Generalization.}




==> Method.tex <==
\section{Methods}
\label{sec:method}
% method -- VR detail
\Eve{move this to method section} 

% ASSUMPTION: One-step Gradient Descent (GD) federated Setting
\begin{assumption}[One-step Gradient Descent (GD) federated Setting]
\label{asp:one-GD}
Assume that the local agents communicate with the central server for $P$ rounds, for each round of local training. Denote that at the end of the $p-$th round of local training, the local model of the $k-$th agent is $h_S^{(k),p}$ and the aggregated model is $h_S^{(0),p}$. $h_S^{(0),0}$ is the initialization of all local models at the first round of training. Correspondingly denote the weights of the models as $w_{h,S}^{(i),p}$, $i\in\{0\}\bigcup [K]$. For each round of local training, the agents do one step GD: 
\begin{align*}
    w_{h,S}^{(i),p} = w_{h,S}^{(0),p-1} - \lambda^{(i),p}\cdot \sE_{(x,y)\sim \gD_S^{(i)}}\big[\nabla_{w}l(h(x,w),y)\big|_{w = w_{h,S}^{(0),p-1}}\big],
\end{align*}
where $\lambda^{(i),p}$ is the learning rate of agent $(i)$ at round $p$.
\end{assumption}

% ASSUMPTION: $\alpha-$Lipschitz Continuous Gradient
\begin{assumption}[$\alpha-$Lipschitz Continuous Gradient]
\label{asp:ltz-grad}
Assume that $l:\gW_h\times\gP_{\gX\times\gY}\to \sR_+$ has the following properties: (1)$ l$ is convex w.r.t. $w_{h}$; (2) $l$ is differentiable w.r.t. $w_{h}$ everywhere; (3) $l$ have an $\alpha$-Lipschitz continuous gradient w.r.t. $w_{h}$ for some $\alpha>0$.  
\end{assumption}


%lemma: federated Round-wise upper bound
\begin{lemma}[Round-wise federated upper bound]
\label{lem:round-ub}
With Assumption \ref{asp:one-GD} and \ref{asp:ltz-grad}, define the domain-wise expected Jacobian matrix of loss $l$ w.r.t $w_h$ as $J_l^{(i)}(w'):= \sE_{(x,y)\in \gD_S^{(i)}} \nabla_{w} l(h(x,w_h),y)\big|_{w_h = w'}$. Suppose the learning rates of all agents at round $p$ are the same: $\lambda^{(i),p} = {\lambda}^{p},\forall i\in[K], p\in[P]$. 
\begin{align*}
    L_{\gD_S}(h_S^{(0),p+1})\leq L_{\gD_S}(h_S^{(0),p})
    -
    \beta_1({\lambda}^{p+1})\cdot
    \|J_l^p\|_2^2 + 
     \beta_2({\lambda}^{p+1})\cdot
    \sigma^2_{J,p}
\end{align*}
where $\beta_1(\lambda) := {\lambda} - \beta_2(\lambda)$; 
$\beta_2(\lambda) := \frac{\alpha{\lambda}^2}{2}$; $J_l^p:= \sE_{i\in[K]}J_l^{(i)}(w_{h,S}^{(i),p})$; 
$\sigma^2_{J,p} :=\sE_{i\in [K]} \|
J_l^{(i)}\big(w_{h,S}^{(0),p}\big)\|_2^2 - \|
J_l^p\|_2^2
$,
\end{lemma}

\textit{Proof is provided in Appendix.}\\\\
\textbf{Interpretation.} The LHS is the loss of the federated model at round $p+1$, which is upper bounded by three terms on the RHS:
\begin{itemize}
% term 1
\item Term 1: $L_{\gD_S}(h_S^{(0),p})$ is the federated loss from the last round. The smaller this term is, the tighter the upper bound is.
% term 3
\item Term 3 $ 
     \beta_2({\lambda}^{p+1})\cdot
    \sigma^2_{J,p}$: the key item is $\sigma^2_{J,p}$, which measures the variance of local gradients across all nodes, since
\begin{align*}
 \sigma^2_{J,p} &:=\sE_{i\in [K]} \|
J_l^{(i)}\big(w_{h,S}^{(0),p}\big)\|_2^2 - \|
J_l^p\|_2^2\\
&= \sE_{i\in [K]} \|
J_l^{(i)}\big(w_{h,S}^{(0),p}\big)\|_2^2 - \|
\sE_{i\in [K]} J_l^{(i)}\big(w_{h,S}^{(0),p}\big)\|_2^2   
\end{align*}
The smaller this term is, the tighter the upper bound is.

$\beta_2({\lambda}^{p+1})=\frac{\alpha(\lambda^{p+1})^2}{2}>0$ is a positive weight determined by the round-wise learning rate and Lipschitz constant of the loss gradient.
% term 2
\item Term 2 $-
    \beta_1({\lambda}^{p+1})\cdot
    \|J_l^p\|_2^2$: the key item is $\|J_l^p\|_2^2:=\|
\sE_{i\in [K]} J_l^{(i)}\big(w_{h,S}^{(0),p}\big)\|_2^2$, which measures the $l2-$norm of expected Jacobian across all nodes. As intuition, a large Jacobian norm leads to a fast drop in the round-wise loss. 

However, we should pay attention to a possible negative $\beta_1({\lambda}^{p+1})$, in which case the upper bound becomes loose and fails to indicate that the federated loss decreases along with rounds. 

To avoid this case, we look into the solution to $\beta_1(\lambda^{p+1}):= {\lambda^{p+1}} - \frac{\alpha(\lambda^{p+1})^2}{2}>0$, which gives $\alpha < \frac{2}{\lambda^{p+1}}$, therefore, $ \|H_l^p\|_2^2 \leq \alpha^2 < \frac{4}{(\lambda^{p+1})^2}$, where $H_l^p$ is the averaged Hessian of $l$ at round p. The number of trainable parameters of model $h$ is $|w_h|$ ($|\cdot|$ denotes cardinality), then the averaged Hessian norm projected to each index follows $ \frac{\|H_l^p\|_2^2}{|w_h|} < \frac{4}{(\lambda^{p+1})^2|w_h|^2}$. In realistic cases, this bound is fairly small, i.e., in a Computer vision task, Adam optimizer typically uses a default learning rate $\lambda = $1e-3, the number of trainable parameters of a ResNet is $|w_h|>$ 1e+7, thus the upper bound of averaged index-wise Jacobian norm should have a scale of 1e-4. To sum up, a constrained averaged Hessian norm over all nodes leads to a tight upper bound.
\end{itemize}



\textcolor{blue}{Apr 6 Eve Update1 Start}

In Lemma \ref{lem:round-ub}, The RHS is a quadratic function w.r.t the learning rate $\lambda$, therefore, the upper bound can be tightened by designing the learning rate at each round. Denote the upper bound for the federated loss at round $p+1$ as $A^{p+1}(\lambda):= L_{\gD_S}(h_S^{(0),p})
    -
    \beta_1({\lambda})\cdot
    \|J_l^p\|_2^2 + 
     \beta_2({\lambda})\cdot
    \sigma^2_{J,p}$. 
For easy writing, we simplify the notation of local Jacobians at round $p$ as $J_l^{(i),p} := J_l^{(i)}\big(w_{h,S}^{(0),p}\big)$ in the rest context.


We discuss the tightness of $A^{p+1}(\lambda)$ w.r.t $\lambda$ as below:
\begin{itemize}
    \item \underline{{$A^{p+1}(\lambda)$ is strictly tight when $\lambda = 0$}}, since Lemma \ref{lem:round-ub} becomes
    $
        L_{\gD_S}(h_S^{(0),p+1})=A^{p+1}(0)= L_{\gD_S}(h_S^{(0),p})
    $.

    \item \underline{If we set $0 < \lambda < \frac{2\cdot\|J_l^p\|_2^2}{\alpha \cdot \sE_i\|J_l^{(i),p}\|_2^2}$, it holds that $A^{p+1}(\lambda) < L_{\gD_S}(h_S^{(0),p})$.} In this case, the upper bound can guarantee that the loss is descending w.r.t federated rounds: $L_{\gD_S}(h_S^{(0),p+1})< L_{\gD_S}(h_S^{(0),p})$.

    \item Denote the optimization of $A^{p+1}(\lambda)$ as ${A^{*,p+1}} := \max_{\lambda}A^{p+1}(\lambda)$, that's ${A^{*,p+1}} = A^{p+1}(\lambda^*)$, where $\lambda^* := \argmax_{\lambda}A^{p+1}(\lambda)$, then we have 
    \underline{
    $
    \lambda^* = \frac{\|J_l^p\|_2^2}{\alpha \cdot \sE_i\|J_l^{(i),p}\|_2^2}$, 
    and 
    $
    A^{*,p+1} =  L_{\gD_S}(h_S^{(0),p})-\frac{\|J_l^p\|_2^4}{2\alpha\cdot \sE_i\|J_l^{p,(i)}\|_2^2}
    $
    }.
    
\end{itemize}

\begin{proposition}[Round-wise federated upper bound optimized over learning rate]
\label{prop:ub-lr}
The best learning rate for Lemma \ref{lem:round-ub} is $\lambda^{*,p+1} = \frac{\|J_l^p\|_2^2}{\alpha \cdot \sE_i\|J_l^{(i),p}\|_2^2}$. The corresponding upper bound is given by
\begin{align*}
    L_{\gD_S}(h_S^{(0),p+1}) \leq L_{\gD_S}(h_S^{(0),p})-\frac{\|J_l^p\|_2^4}{2\alpha\cdot \sE_i\|J_l^{p,(i)}\|_2^2}
\end{align*}

\end{proposition}
\remark Rewrite the second term as $\frac{\|J_l^p\|_2^4}{2\alpha\cdot \sE_i\|J_l^{p,(i)}\|_2^2} = \frac{\|J_l^p\|_2^2}{2\alpha}\cdot
\frac{\|J_l^p\|_2^2}{\sE_i\|J_l^{p,(i)}\|_2^2}$. The multiplier $\frac{\|J_l^p\|_2^2}{\sE_i\|J_l^{p,(i)}\|_2^2}\in[0,1]$, and $\frac{\|J_l^p\|_2^2}{\sE_i\|J_l^{p,(i)}\|_2^2} = 1$ iff $\sigma^2_{J,p} = 0$ (the variance of Jacobians over local nodes is 0), in this ideal case we have the tightest bound
$
L_{\gD_S}(h_S^{(0),p+1}) \leq L_{\gD_S}(h_S^{(0),p})-\frac{\|J_l^p\|_2^2}{2\alpha}
$. 

\textcolor{purple}{\textbf{Technique 1} (choose learning-rate)}: At the start of round $p+1$, the central server broadcast ${\|J_l^p\|_2^2}$ and ${ \sE_i\|J_l^{(i),p}\|_2^2}$. The local nodes then set the learning rate $\lambda^{p+1} = \frac{\|J_l^p\|_2^2}{\alpha \cdot \sE_i\|J_l^{(i),p}\|_2^2}$ for local training. Estimation for $\alpha$ can be inspired by $\alpha \geq \frac{\|J_l(w) - J_l(w')\|}{\|w - w'\|},\forall w, w' $.

\textcolor{purple}{\textbf{Technique 2} (mitigate variance across nodes)}: At the start of round $p+1$, the central server broadcast ${J_l^p}$. The agents then train a regularized objective $L_{\gD_S^{(i)}}(h_S^{(i),p+1}) + \lambda_{J}\cdot\|J_l^{p+1,(i)} - J_l^p\|_2^2$, where $\lambda_{J}$ is the penalty parameter. The theoretical guarantee for this technique is discussed below.

\begin{proposition}[federated upper-bound with regularization]
\label{prop:ub-reg}
    Suppose for each round $p>1$ the agents choose the best learning rate from Proposition \ref{prop:ub-lr}: $\lambda^p = \frac{\|J_l^{p-1}\|_2^2}{\alpha \cdot \sE_i\|J_l^{(i),{p-1}}\|_2^2}$. Suppose $\|J_l^{p,(i)} - J_l^{p-1}\|_2^2\leq \gamma \|J_l^{p-1}\|_2^2, \gamma \in (0,1),\forall i\in[K],1<p\leq P$. Then by one-step GD federated training,
    \begin{align}
    \label{eq:ub-reg}
         L_{\gD_T}(h_T^{(0),P}) 
         \leq L_{\gD_S}(h_S^{(0),1})
         -\frac{1-\gamma-(1-\gamma)^{P}}
         {2\alpha\gamma\cdot(1+\gamma)}\|J_l^1\|_2^2 +d_{\gF}(\gD_S,\gD_T).
    \end{align}
\end{proposition}

\remark RHS decreases as federated round $P$ increases. Given adequate rounds, we have $\lim_{P\to\infty}  L_{\gD_S}(h_S^{(0),P})
\leq L_{\gD_S}(h_S^{(0),1})
         -\frac{1-\gamma}
         {2\alpha\gamma\cdot(1+\gamma)}\|J_l^1\|_2^2 +d_{\gF}(\gD_S,\gD_T)$.


\textcolor{purple}{\textbf{Technique 3} (local Contrastive Learning (CL) w.r.t Jacobian)}: The agents augment their data $x$ by $x'\sim T(x)$, where $T(x)$ is the distribution of transformation based on original data $x$. Denote the population distribution sampled by agent $i$ as $\hat{\gD}_S^{(i)}$. Denote all variables related to augmentation by $\cdot'$. Define $J_l(x,y):= \nabla_w l(h(x,w),y)$. The agent $(i)$ train a regularized objective $L_{\hat{\gD}_S^{(i)}}(h_S^{(i)}) 
+ \lambda_{CL}\cdot\sE_{(x,y) \sim \hat{\gD}_S^{(i)}} \sE_{x'\sim T(x)}\|J_l(x,y)
- J_l(x',y)\|_2^2$. The intuition for CL here is  
\begin{enumerate}
    \item To strengthen the smoothness of the model $l(h(x,w),y)$. By constraining $\|J_l(x,y)
- J_l(x',y)\|_2^2, x'\sim T(x)$, we are decreasing the capacity of $\gH$, so as to expect a decrease in the smoothness factor $\alpha:=\underset{h\in \gH;w,w'\in \gW}{\sup}\frac{\|J_l(w) - J_l(w')\|}{\|w-w'\|}$, and further tighten the bounds (i.e., the bound of Eq. (\ref{eq:ub-reg})).  

\item To learn a better estimation of the ground-truth representation (in this case, ground-truth Jacobian) compared with learning without CL. Below we discuss a toy case where \textit{local CL on Jacobian} can tighten the round-wise federated upper bound.
\end{enumerate}

\textbf{A toy case for local CL on Jacobian}. Recall 
 that ${J}_l^{(i)}:= \sE_{(x,y)\sim \gD_S^{(i)}} \nabla_x(h(x,w),y)$ is the ground-truth local Jacobian. Denote all variables regarding the sampled population as $\hat{\cdot}$. Therefore, the observed Jacobian is denoted by $\hat{J}_l^{(i)}$. Define $\delta^{(i)}:= \hat{J}_l^{(i)} - J_l^{(i)} $ as the deviation between the observed and ground-truth Jacobian of agent $i$. Suppose $\sE_{i}\delta^{(i)} = 0$. Suppose that training with contrastive learning can give ground-truth Jacobian, that is $\delta^{(i),CL} = 0$ and $\hat{J}_l^{(i),CL} = {J}^{(i)}_l$.

\begin{proposition}
Denote the upper bound in Proposition \ref{prop:ub-lr} (without CL) as $\hat{U}^{p+1}:=L_{\hat{\gD}_S}(\hat{h}_S^{(0),p})-\frac{\|\hat{J}_l^p\|_2^4}{2\alpha\cdot \sE_i\|\hat{J}_l^{p,(i)}\|_2^2}$, and the upper bound with CL as $\hat{U}^{p+1,CL}:=L_{\hat{\gD}_S}(\hat{h}_S^{(0),p,CL})-\frac{\|\hat{J}_l^{p,CL}\|_2^4}{2\alpha_{CL}\cdot \sE_i\|\hat{J}_l^{p,(i),CL}\|_2^2}$. In the toy case above, suppose CL is applied only at round $p$, by one-step GD, we have
\begin{align*}
    \hat{U}^{p+1,CL} <  \hat{U}^{p+1}. 
\end{align*}
\end{proposition}


\textcolor{blue}{Apr 6 Eve Update1 End}


% Theorem: Multi-round transfer upper bound
\begin{theorem}(Multi-round transfer upper bound)
\label{thm:Mrd-tdf-fed-ub}
\begin{align*}
    L_{\gD_T}(h_T^{(0),P})\leq L_{\gD_S}(h_S^{(0),0})
    -\sum_{p=0}^{P-1}
    \beta_1({\lambda}^{p+1})
    \|J_l^p\|_2^2 + \sum_{p=0}^{P-1}
     \beta_2({\lambda}^{p+1})
    \sigma^2_{J,p} + d_{\gF}(\gD_S,\gD_T).
\end{align*}
\end{theorem}

\textit{Proof is obvious by combining Lemma \ref{lem:gen-tsf-ub} and \ref{lem:round-ub}.}\\\\
\textbf{Interpretation.} Terms are all mentioned in Lemma \ref{lem:gen-tsf-ub} and Theorem \ref{thm:gen-tsf-fed-ub}.\\\\
\textbf{Sufficient Conditions.} From Lemma \ref{lem:round-ub} and Theorem \ref{thm:Mrd-tdf-fed-ub}, we have the following sufficient conditions during federated pre-training to tight the upper bound and reasonably expect a lower transfer loss:
\begin{itemize}
    \item A good initial model with low loss; (In practice, we can randomly sample a set of initial models and choose the one with the lowest initial loss)
    \item Proper penalization on the Hessian norm of the whole model. (In practice, we can use Jacobian regularization in practice)
    \item Proper penalization on the variance of Jacobian across all nodes (In practice, we can \textcolor{red}{design a \textit{contrastive-Jacobian learning}}, each agent penalizes the Jacobian variance between original data and augmented data.)
\end{itemize}


\begin{theorem}[Hessian-related upper bound]
Assume that $l:\gW_h\times\gP_{\gX\times\gY}\to \sR_+$ is convex w.r.t. $w_{h}$ and twice-differentiable everywhere.
\end{theorem}
\Eve{todo: add a theorem where the local training is one-step GD. consider Hessian.}

\begin{theorem}[finit sample upper bound]
\end{theorem}
\Eve{todo: do the finite-sample version for all theorems above}



 
\begin{algorithm}[H]
\caption{Transferable Federated Learning \textcolor{blue}{Eve Mar 6 Update2}}\label{alg:cap}
\begin{algorithmic}
\Require Agent number $K$, Federated round $P$, Local data sets $\{\hat{D}_S^{(i)}\}_{i\in [K]}$.
% \Ensure $y = x^n$
\State Randomize local models $h_S^{(i),0}$;
\State $p\gets 1$ \Comment{round index initialization.}
\State $k\gets 1$ \Comment{agent index initialization.}
\State $S_{\alpha}\gets \emptyset$ \Comment{$(J,w_h)$-pair storage initialization.}
\While{$k \leq K$}
\State Agent (k) augments its data.
\State Agent (k) applies Contrastive Learning (CL) on Jacobian and obtains $h_S^{(i),1}, J_l^{(i),1}$.
\State{$k\gets k+1$}
\EndWhile
\State Server (0) collects $h_S^{(i),1}, J_l^{(i),1}$ and adds all the $(J,w_h)$ pairs into $S_\alpha$.
\State Server (0) estimates $\hat{\alpha} :=
\underset{(J,w),(J',w')\in S_\alpha}{\sup}\frac{\|J-J'\|}{\|w-w'\|}$.
\State Server (0) computes $h_S^{(0),1}, J_l^{1}$ and $\lambda^2:= \frac{\|J_l^1\|_2^2}{\hat{\alpha} \cdot \sE_i \|J_l^{(i),1}\|_2^2}$. 
\State{$p\gets p+1$}
\State{$k\gets 1$}
\While{$p\leq P$}
\State Server (0) broadcasts $h_S^{(0),p-1}, \lambda^p$ and $J_l^{p-1}$.
\While{$k\leq K$}
\State $h_S^{(k)}\gets h_S^{(0),p-1}$
\State $\lambda^{(k),p}\gets \lambda^p$ \Comment{Technique 1: choose learning rate}
\State Agent (k) augments its data $x'\sim T(x)$
\State Agent (k) obtains $h_S^{(k),p}$ by training a loss $L_{\hat{\gD}_S^{(k)}}(h_S^{(k)})+\omega_{CL}\cdot \sE_{(x,y)\sim\hat{\gD}_S^{(i)}} \sE_{x'\sim T(x)} \|J_l(x,y) - J_l(x',y)\| +\omega_{J}\cdot\|J_l^{(i)} - J_l^{p-1}\|$ 
\Comment{Technique 2 and 3}
\State{$k\gets k+1$}
\EndWhile
\State Server (0) collects $h_S^{(i),p}, J_l^{(i),p}$ and adds all the $(J,w_h)$ pairs into $S_\alpha$.
\State Server (0) estimates $\hat{\alpha} :=
\underset{(J,w),(J',w')\in S_\alpha}{\sup}\frac{\|J-J'\|}{\|w-w'\|}$.
\State Server (0) computes $h_S^{(0),p}, J_l^{p}$ and $\lambda^{p+1}:= \frac{\|J_l^p\|_2^2}{\hat{\alpha} \cdot \sE_i \|J_l^{(i),p}\|_2^2}$. 
\State{$p\gets p+1$}
\State{$k\gets 1$}
\EndWhile
\end{algorithmic}
\end{algorithm}


==> ProblemFormulation.tex <==
\section{Problem Formulation}

\textbf{Preliminaries and Notations.} We denote the input space as $\gX$, the output space as $\gY$, the feature space as $\gZ$. Let a feature extractor be $f\in \gF$ and a fine-tuning function be $g\in \gG$, where $\gF, \gG$ are function classes. Denote $\gW_f$ and $\gW_g$ as the parameter spaces for $f$ and $g$. Given a feature extractor $f(\cdot, \cdot):  \gX \times\gW_f \rightarrow \gZ$ and a fine-tuning function $g(\cdot, \cdot):  \gZ \times\gW_g \rightarrow \gY$, the full model is $h: = g\circ f$, therefore, we have $h(\cdot, \cdot):\gX \times \gW_h \rightarrow \gY$, where $\gW_h = \gW_g \times \gW_f$ is the parameter space for $h$. Given a loss function $l(\cdot,\cdot):\gY \times \gY \rightarrow \sR$, the population loss based on data distribution $\gD \in \gP_{\gX \times \gY}$ (where $\gP_{\gX \times \gY}$ is the class of all possible distributions for pair (x,y)) and a model $h$ is defined as {\color{blue} (Is $\gP_{\gX \times \gY}$ the class of all distributions? (eve: check))}
\begin{align*}
    L_{\gD}(h):= \sE_{(x,y)\sim \gD}l(h(x,w_h),y).
\end{align*}




{\color{blue} Should the left-hand side also depend on $w_h$? (eve: $w_h$ is the parameter of h, for simplicity, on the LHS I only wrote $\gD$ and $h$, which will include information on $x,y,w_h$.)}

In a Transfer Learning (TL) task, we conduct $K$-agent federated learning on the source domain and then fine-tune the pretrained federated model on the target domain. Denote the data distribution of the source domain as $\gD_S$, which is the joint distribution of all local domains $\{\gD_S^{(k)}\}_{k\in[K]}$. The loss on the source domain is the federated loss
\begin{align*}
    L_{\gD_S}(g\circ f) =  \frac{1}{K}\sum_{i=1}^K L_{\gD_S^{(i)}}(g\circ f).
\end{align*}
{\color{blue} The expectation should be replaced by sum? (eve: checked)}


Denote the index of local agents by $\{(k)\}_{k=1}^K$ and that of the central server as $(0)$. Denote the pre-trained federated model as $h^{(0)}_{S} = g^{(0)}_{S}\circ f^{(0)}_{S}$ and the individual models as $h^{(k)}_{S} = g^{(k)}_{S}\circ f^{(k)}_{S}, k\in[K]$. {\color{blue} From here you started to index the functions $f$ and $g$ by $f_S$, $g_S$, $g_T$. You should explain what these new notations refer to. (eve: check)} Correspondingly denote the model weights as $w_{\phi,S}^{(k)}$, where $\phi\in\{h,f,g\}$, $k\in \{0\}\bigcup [K]$. In the case of FedAVG (the ubiquitous conventional FL algorithm), we have
\begin{align*}
    w_{\phi,S}^{(0)} = \frac{1}{K}\sum_{i=1}^K w_{\phi,S}^{(k)}.
\end{align*}
{\color{blue}I guess expectation should be replaced by sum and $i$ should change to $k$. (eve: check)}

When adapting the model on the target domain, the pre-trained feature extractor $f_S^{(0)}$ is typically fixed~\cite{weiss2016survey}, {\color{blue} (Is this an assumption?) eve: check} therefore, the target loss given a fine-tuning function $g$ is $L_{\gD_T}(g\circ f_S^{(0)})$. By fine-tuning $g$, we look for
\begin{align*}
    g_T = \arg\inf_{g\in \gG} L_{\gD_T}(g\circ f_S^{(0)}).
\end{align*}
The performance on the target domain is evaluated by $L_{\gD_T}(g_T\circ f_S^{(0)})$.

The question is: \textcolor{red}{What are sufficient conditions for a federated pre-training mechanism, such that the pre-trained model transfers well to the target domain (equivalently, $L_{\gD_T}(g_T\circ f_S^{(0)})$ is small)?}

\begin{definition}[Definition 2.3 in \cite{xu2022adversarially}] 
Given a fine-tuning
function class $\gG$, a feature extractor function class $\gF$ and
distributions $\gD_S$, $\gD_T \in \gP_{\gX\times\gY}$, the ($\gG$, $\gF$)-divergence
between $\gD_S, \gD_T$ is
\begin{align*}
d_{\gG,\gF} (\gD_S, \gD_T ) := \sup_{f\in\gF}
|\inf_{g\in\gG}L_{\gD_S}(g \circ f) -
\inf_{g\in\gG}L_{\gD_T}(g \circ f)|.    
\end{align*}
\end{definition}
\remark Since practically $\gG$ is typically fixed and clear, so we will simplify the notation as $d_\gF$ in the rest context. the pseudo-matrix satisfies properties as follows:
\begin{itemize}
\item (Symmetry.) $d_{\gG,\gF}(\gD_S,\gD_T) = d_{\gG,\gF}(\gD_T,\gD_S)$.
\item (Triangle Inequality {\color{blue} what is $\gH$ here? (eve: check)}.) $d_{\gG,\gF}(\gD_S,\gD_T) \leq d_{\gG,\gF}(\gD_S,\gD') + d_{\gG, \gF}(\gD',\gD_T)$.
\item (Zero Property.) $d_{\gG,\gF}(\gD,\gD) = 0$.
\end{itemize}

\begin{lemma}[Theorem 2.5 in \cite{xu2022adversarially}]
\label{lem:gen-tsf-ub}
Given pre-training on the source domain and fine-tuning on the target domain,
$\forall \gD_S, \gD_T \in \gP_{\gX\times\gY}$ we have
\begin{align*}
    L_{\gD_T}(g_T \circ f_S^{(0)}) \leq L_{D_S} (g_{S}^{(0)}  \circ f_{S}^{(0)} ) + d_{\gG,\gF} (\gD_S,\gD_T ).
\end{align*}
\end{lemma}

\begin{definition}($\gH$-pseudo-matrix.)
Given distributions $\gD_S, \gD_T\in \gP_{\gX \times \gY}$, model function class $\gH$ and loss function $L$, the $\gH$-pseudo-matrix between $\gD_S$ and $\gD_T$ is  
\begin{align*}
    d_{\gH}(\gD_S,\gD_T):= \inf_{h\in \gH}|L_{\gD_S}(h) -L_{\gD_T}(h) |.
\end{align*}
\remark This is a measurement of domain divergence depending not only on the input distribution (as the conventional measurement does) but also on the label distribution and loss function. It satisfies properties as follows:
\begin{itemize}
\item (Symmetry.) $d_{\gH}(\gD_S,\gD_T) = d_{\gH}(\gD_T,\gD_S)$.
\item (Triangle Inequality.) $d_{\gH}(\gD_S,\gD_T) \leq d_{\gH}(\gD_S,\gD') + d_{\gH}(\gD',\gD_T)$.
\item (Zero Property.) $d_{\gH}(\gD,\gD) = 0$.
\end{itemize}


\Eve{todo: (1) check if others already define this, if so, cite it; (2) if not, discuss its
 difference from previous domain divergence measurements, i.e., H-divergence.}
\end{definition}



==> evaluation.tex <==
\section{Evaluation (for ourselves to check)}

\Eve{Overall, it's a relatively low-risk project, worth trying during summer.}

\subsection{Feasibility}
Compared with defense paper (usually a defense mechanism inspired/validated by theory), attack paper has a higher requirements for experiment (i.e., the attack should work across various data set to avoid task-bias, which is usually not questioned in the defense paper), since attack paper 1) focuses on the experiment results (successfully poison an existing model) and 2) can hardly involve theory. 

Therefore, the concerns about this project mainly lie in the \underline{experiment design} including:
\begin{itemize}
    \item No mature framework (\Eve{ \href{https://github.com/flint-xf-fan/Byzantine-Federeated-RL}{link for code of~\cite{fan2021fault}}})
    \item RL NN hard to tuning
    \item What data set is "good" (how to convince the review it's good)? (\Eve{Fan, Xiaofeng, et al. \cite{fan2021fault} used the RL benchmark, we could take it for reference but note that it's a defense paper that may enjoy lower requirements for experiments.})
\end{itemize}



\subsection{Importance}
\begin{itemize}
    \item \underline{Attack Method}: Besides the FL attack introduced by~\cite{bhagoji2019analyzing}, we'd better also exquisitely leverages the RL attack~\cite{pinto2017robust}~\cite{uther1997adversarial} which involves error aggregation; (convince the reviewer that it's not "easy adaption")
    \item \underline{Attack target}: the target that we choose to attack doesn't have local step, therefore, may not represent RFL framework, however, since it's published (in NeurIPS), we can still use it as our attack target temporarily; After that, we may find more attack targets in the published application papers (IoT, Auto-drive, etc.)
\end{itemize}

\Eve{Other general concerns: Paper writing: make sure to clarify the logic and highlight the importance.}






